Cross-Lingual Dialogue Dataset Creation via Outline-Based Generation

Multilingual task-oriented dialogue (ToD) facilitates access to services and information for many (communities of) speakers. Nevertheless, the potential of this technology is not fully realised, as current datasets for multilingual ToD - both for modular and end-to-end modelling - suffer from severe limitations. 1) When created from scratch, they are usually small in scale and fail to cover many possible dialogue flows. 2) Translation-based ToD datasets might lack naturalness and cultural specificity in the target language. In this work, to tackle these limitations we propose a novel outline-based annotation process for multilingual ToD datasets, where domain-specific abstract schemata of dialogue are mapped into natural language outlines. These in turn guide the target language annotators in writing a dialogue by providing instructions about each turn's intents and slots. Through this process we annotate a new large-scale dataset for training and evaluation of multilingual and cross-lingual ToD systems. Our Cross-lingual Outline-based Dialogue dataset (termed COD) enables natural language understanding, dialogue state tracking, and end-to-end dialogue modelling and evaluation in 4 diverse languages: Arabic, Indonesian, Russian, and Kiswahili. Qualitative and quantitative analyses of COD versus an equivalent translation-based dataset demonstrate improvements in data quality, unlocked by the outline-based approach. Finally, we benchmark a series of state-of-the-art systems for cross-lingual ToD, setting reference scores for future work and demonstrating that COD prevents over-inflated performance, typically met with prior translation-based ToD datasets.

==> notes.tex <==
\begin{table}
\footnotesize{
\begin{tabularx}{0.9\textwidth}{XXX}
\hline  & \bf Dev & \bf Test \\ \hline
Domains & 8  & 8  \\
Dialogues & 92  & 102 \\
Turns & 1138 & 1352 \\
\bottomrule
\end{tabularx}}
\caption{Data statistics.}
\label{tab:datastats}
\end{table}

\begin{table*}
\footnotesize{
\begin{tabularx}{0.9\textwidth}{X}
\toprule
\textbf{USER} \\ 
\hline
\textit{Express the desire to search for roundtrip flights for the trip}\\
the name of the airport or city to arrive at : Seattle\\
the company that provides air transport services : American Airlines\\
\hline
\foreignlanguage{russian}{Мне нужно найти рейс в Ставрополь и обратно авиакомпании S7.}\\
\hline
the name of the airport or city to arrive at : \foreignlanguage{russian}{Ставрополь}\\
the company that provides air transport services : S7\\
\hline \textbf{ASSISTANT} \\ \hline
Inform the user that you found 1 such option(s)	
Offer the following option(s): 	
the company that provides air transport services :  American Airlines\\
departure time of the flight flying to the destination :  7:35 am	\\
not a direct flight	\\
departure time of the flight coming back from the trip :  4:15 pm	\\
the total cost of the flight tickets :  \$343	\\
\hline
\foreignlanguage{russian}{Найден 1 рейс авиакомпании S7 с пересадкой, вылет в 7:35, возвращение в Москву в 16:15. Стоимость билетов 6845 рублей.}\\
\hline
the company that provides air transport services :  S7\\
departure time of the flight flying to the destination :  07:35\\
departure time of the flight coming back from the trip :  16:15\\
the total cost of the flight tickets :  \foreignlanguage{russian}{6845 рублей}\\

\bottomrule
\end{tabularx}}
\caption{Example of prompt-based dialogue generation and slot filling in Russian.}
\label{tab:prompt_examples}
\end{table*}
